On incompressible flows in discrete networks and Shnirelman's inequality

Let $f$ and $g$ be two volume-preserving diffeomorphisms on the cube $Q=[0,1]^{\nu}$, $\nu \geq 3$. We show that there is a divergence-free vector field $v \in L^1((0,1);L^p(Q))$ such that $v$ connects $f$ and $g$ through the corresponding flow and $\Vert v \Vert_{L^1_t L^p_x} \leq C_{p,\nu} \Vert f- g \Vert_{L^p_x}$. In particular we show Shnirelman's inequality, cf. [Shnirelman, Generalized fluid flows, their approximation and applications (1994)], for the optimal H\"older exponent $\alpha =1$, thus proving that the metric on the group of volume-preserving diffeomorphisms of $Q$ is equivalent to the $L^2$-distance. To achieve this, we discretise our problem, use some results on flows in discrete networks and then construct a flow in non-discrete space-time out of the discrete solution.

==> appunti.tex <==
\item Let $\sigma$ be a permutation and $\psi_{\sigma}$ be the corresponding map on the tiling $\Rcal_N$. Then there is $\varepsilon_0>0$ such that for all $\varepsilon < \epsilon_0$ there is a map $f_{\varepsilon} \in \mathcal{D}(\Omega)$ such that for all $1 \leq p < \infty$ 
        \[
        \Vert f_{\varepsilon} - \psi_{\sigma} \Vert_{L^p} \leq C(p) \varepsilon
        \]
        and a smooth flow $\phi \colon [0,1] \to \mathcal{D}(\Omega)$ from $\id$ to $f_{\varepsilon}$ such that
        \[
         \Vert \dot{\phi} \Vert_{L^q_t L^p_x} \leq \Vert \psi_{\sigma} - \id \Vert_{L^p_x}, \quad \forall 1 \leq p,q \leq \infty.
        \]
    \end{enumerate}
